First order of the renewal covering of the natural numbers

This paper introduces a new type of covering process that covers the set of natural numbers using renewal processes as objects. Inspired by the behavior of prime numbers, the model in each step finds the smallest vacant point, $k$, and place, starting in $k$, a renewal process with a step distribution given by a geometric random variable with parameter $\frac{1}{k}$. The model depends on its entire past, and small perturbations in its initial value can lead to very different outcomes. Here, we expose a technique that finds the first-order limit behavior for the number of objects placed until $n$, which exhibits intriguing similarities to prime number distributions, having a concentration around $n\log{n}$.

==> lixo.tex <==

to construct the element $P_{n+1}$, proce

Start by choosing $P_1=2$ almost surely, then for each $k\in\left\{P_1+1,P_1+2,\cdots \right\}$ sample an independent Bernoulli $\xi_k^1$ with parameter $\frac{1}{P_1}=\frac{1}{2}$.  Define the set of \textbf{random multiples} of $P_1$, or equivalently the renewal set, as $\mathcal{M}_1=\{k> P_1: \xi_k^1=1\}$. Notice that with probability one there exists a minimum element in the set $\{k>P_1\}\setminus\mathcal{M}_1$, such minimum element will be $P_2$, moreover we have $P_2-P_1\sim \G{\left(1-\frac{1}{2}\right)}$. In general, with a value of $P_j$, for each natural number $k\in\left\{P_j+1,P_j+2,\cdots\right\}$, sample an independent Bernoulli $\xi_k^j$ with parameter $\frac{1}{P_j}$. Define the set of random multiples of $P_j$ as $\mathcal{M}_j=\{k> P_{j}: \xi_k^j=1\}$, then take $P_{j+1}$ to be the minimum element of $\{k>P_j\}\setminus\bigcup_{k=1}^j \mathcal{M}_k$. In particular, $P_j-P_{j-1}\sim \G{\prod_{k=1}^j\left(1-\frac{1}{P_j}\right)}$. 

\section{Second term in the law of large numbers}\label{sec:law2}

Assume $x$ to be large enough so that $\frac{(1+a)\log{\log{x}}}{\log{x}}<1$, then: 

\begin{align*}
    &\int_x^{x^\beta}dy\exp\left\{\int_x^y \frac{dt}{t\log{t}+(1+a)t\log{\log{t}}}\right\}\\
    &=\int_x^{x^\beta}dy\exp\left\{\int_x^y \frac{dt}{t\log{t}\left(1+(1+a)\frac{\log{\log{t}}}{\log{t}}\right)}\right\}\\
    &=\int_x^{x^\beta}dy\exp\left\{\int_x^y \frac{dt}{t\log{t}} \sum_{k=0}^{\infty} \left((-1-a)^k \left(\frac{\log{\log{t}}}{\log{t}}\right)^k\right) \right\}\\
    &\leq \int_x^{x^\beta}dy\exp\left\{\int_x^y \frac{dt}{t\log{t}} \sum_{k=0}^{2} \left((-1-a)^k \left(\frac{\log{\log{t}}}{\log{t}}\right)^k\right) \right\}\\
    &= \int_x^{x^\beta}dy\exp\left\{\int_x^y dt\left( \frac{1}{t\log{t}} - (1+a) \frac{\log{\log{t}}}{t\ln^2{\left(t\right)}} +(1+a)^2  \frac{\left(\log{\log{t}}\right)^2}{t\ln^3{\left(t\right)}}\right)\right\}\\
     &= \int_x^{x^\beta}dy\exp\left\{ \begin{aligned}  
     &-\log{\log{x}}+\log{\log{y}} \\&- (1+a)\left(\frac{1+\log{\log{x}}}{\log{x}} -\frac{1+\log{\log{y}}}{\log{y}}\right)\\
     &+ \frac{(1+a)^2}{4}\frac{1+2\log{\log{x}}+2\left(\log{\log{x}}\right)^2}{\ln^2\left(x\right)}\\&- \frac{(1+a)^2}{4}\frac{1+2\log{\log{y}}+2\left(\log{\log{y}}\right)^2}{\ln^2\left(y\right)}
     \end{aligned}\right\}\\
     &\leq \int_x^{x^\beta}dy\frac{\ln{y}}{\ln{x}}\left(1+ (1-\delta)\left( \begin{aligned}  
     &- (1+a)\left(\frac{1+\log{\log{x}}}{\log{x}} -\frac{1+\log{\log{y}}}{\log{y}}\right)\\
     &+ \frac{(1+a)^2}{4}\frac{1+2\log{\log{x}}+2\left(\log{\log{x}}\right)^2}{\ln^2\left(x\right)}\\&- \frac{(1+a)^2}{4}\frac{1+2\log{\log{y}}+2\left(\log{\log{y}}\right)^2}{\ln^2\left(y\right)}
     \end{aligned} \right)\right)\\
     &= \int_x^{x^\beta}dy\frac{\ln{y}}{\ln{x}}\left(1+ (1-\delta)\left( \begin{aligned}  
     &- (1+a)\frac{1+\log{\log{x}}}{\log{x}} \\
     &+ \frac{(1+a)^2}{4}\frac{1+2\log{\log{x}}+2\left(\log{\log{x}}\right)^2}{\ln^2\left(x\right)}
     \end{aligned} \right)\right)\\
     &\quad\text{    }\quad \, +  \int_x^{x^\beta}dy \frac{ (1-\delta)}{\ln{x}}\left( \begin{aligned}  
     & (1+a)\left(1+\log{\log{y}}\right)\\
     &- \frac{(1+a)^2}{4}\frac{1+2\log{\log{y}}+2\left(\log{\log{y}}\right)^2}{\ln\left(y\right)}
     \end{aligned} \right)\\
\end{align*}



\begin{Rmk}
    The arguments presented in this paper stop working in the third-order term that might be supported in the real line. However, because of the numerical studies, specifically using equation \eqref{eq:DursattRosserbound}, we suspect that $Z$ is the Mandelbrot-Shepp distribution with support in $[0,1]$,  commonly found in covering problems; see \cite{AMC2024}. Some explanation of the conjecture together with some comments about the Crammer hypothesis is given during the proofs of the theorems. 
\end{Rmk}


   
   %more realistic, consider the process below $(1+a)n\log{n}$. Due to estimation of the value of $\lambda_n$, according to Karamatha's conditions \eqref{eq:conditions2boa}, one gets a logarithmic bound. Then, according to the evaluation carried out in Proposition \ref{Prop:LargeDeviationGeoindpendent} generalization proof, in equation \eqref{eq:Geometricdifferenceboundfinite}, the value for the increment will for every $n$ large be  be of size less than $\ln^2(n)$. Moreover, due to condition \eqref{eq:conditions1boa}, it is possible to control the sum $    \sum_{k=1}^{n^{\beta}} \lambda_{k}^{-1}$  by controlling the value of $P_n$. Therefore, instead of doing the proof in $(1+a)n\log{n}$ to $(1+2a)(n\log{n})$, it is possible to find $\eta>0$ small, and look to starting points in between $(1+a+\eta)n\log{n}$, to guarantee both $\sum_{k=1}^n \lambda_n^{-1}$ and $P_n$ larger than $(1+a)n\log{n}$, therefore, choosing a smaller value of $\delta$, and correcting the bound \eqref{eq:boundintheonion} to starting in $(1+a+\eta)x\ln{x}$ stills not hit $(1+2a)x\ln{x}$. 
\subsection{Returning to the tightness}

This section, we are interesting to show that $\lambda_n$ is not just slowly varying, it belongs to a sharper subset of slowly varying functions. For this, we are going to go back to the proof of tightness of the sequence $\lambda_n$, but known knowing that $P_n> (1-\delta)\frac{n}{\lambda_n}$.

Define the set of \textbf{sharp slowly varying sequences}, as: 
\begin{align*}
    \SV^{(s)}=\left\{(\gamma_k)_k: \begin{aligned}
        \lim_{x\to \infty} \gamma(x)=\infty, &\,\text{ and }\\
         \forall t>0, \,\exists C_t>0 \text{ s.t. }& 1-\frac{C_t}{\gamma(x)}\leq \frac{\gamma(xt)}{\gamma(x)}\leq 1+\frac{C_t}{\gamma(x)}
    \end{aligned}\right\}. 
\end{align*}In essence, this subset controls the  velocity that the ratio converges to one. One example of function that belongs to $\SV^{(s)}$ is $\log(x)$ with constant $C_t=\log{t}$. Another example, now of a slowly varying function that do not belongs to $\SV^{(s)}$,  is $\log^2(x)$. The condition that $\lim_{x\to \infty} f(x)=\infty$ is only used to make the bound in the slowly varying ratio acceptable. 

\begin{Lem}\label{Lem:lambdaslowv1}
 The sequence $(\lambda^{-1}_k)_k\in \SV^{(s)}$ with probability one. Moreover, for every $\e>0$, $\delta>0$ and $t>0$, there exists $x_0=x_0(\e,\delta,t)$ such that: 
\begin{align}\label{eq:quantitativelambdaslow1}
    \P{1-\frac{(t^{-1}-1)(1-\delta)\lambda(x)}{(1+\delta)} \leq \frac{\lambda^{-1}(xt)}{\lambda^{-1}(x)}\leq 1+\frac{(1-t^{-1})\lambda(x)}{(1-\delta)}, \, \forall x>x_0}>1-\e. 
\end{align}
\end{Lem}
\begin{proof}
    For $t>1$, we have by equation \eqref{eq:elavaivoltar} that:  
    \begin{align}
    1\leq\frac{\lambda^{-1}(xt)}{\lambda^{-1}(x)}\leq \exp\left\{\frac{xt(1-t^{-1})}{P_{\lceil xt\rceil}}\right\}. \label{eq:boundintherateoflambdaslow1}
    \end{align} Therefore, by Corollary \ref{Cor:concentrationfirt} and the monotonicity of $\lambda(x)$, for every $\e>0$ and  $\delta>0$, there exists $x_1=x_1(\e,\delta)$ such that for all $x>x_1$, we have that $P_x>(1-\delta)\frac{x}{\lambda_x}$ and $\frac{\lambda(xt)}{1-\delta}<\frac{\lambda(x)}{1-\delta}<1$ occurs with probability greater than $1-\e$. Then, since $e^{x/2}\leq 1+x$ if $x<1$, we get that:
    \begin{align}
    \P{1\leq\frac{\lambda^{-1}(xt)}{\lambda^{-1}(x)}\leq 1+\frac{(1-t^{-1})\lambda(x)}{(1-\delta)}, \forall x>x_1}>1-\e. \label{eq:boundintherateoflambdaslow1}
    \end{align}
    
    Now, for $t\in (0,1)$, we get that:
    \begin{align*}
    1\geq\frac{\lambda^{-1}(xt)}{\lambda^{-1}(x)}\geq \exp\left\{-\frac{xt(t^{-1}-1)}{2P_{\lceil xt\rceil}}\right\}. 
    \end{align*} Witch implies there exists $x_2=x_2(\e,\delta)$ such that:
    \begin{align}
    \P{1\geq\frac{\lambda^{-1}(xt)}{\lambda^{-1}(x)}\geq 1-\frac{(t^{-1}-1)(1-\delta)\lambda(x)}{2(1+\delta)}, \forall x>x_2}>1-\e. \label{eq:boundintherateoflambdaslow1}
    \end{align} To finish the proof, just take $x_0(\e,\delta,t)$ to be equal to $x_2$ if $t\in(0,1)$ or otherwise, $x_1$. 
\end{proof}

In particular, we have that when using Karamatha's theorem, we can make the $\sum_{k=1}^n \frac{1}{\lambda_k}$ closer to the value of $\frac{x}{\lambda_k}$. That is:


\subsection{Integral and Differential equations}

As a conclusion of the Lemma \ref{Lem:firstconcentration}, for some $c>0$ we are trying to give quantitative informations about the sequence $\lambda(x)$ that satisfies:
\begin{align*}
    |\sum_{k=1}^n \frac{1}{\Lambda(x)}- n\frac{1}{\lambda_n} +c(x)n|=0
\end{align*}Thus, lets find the functions $f$ such that:
\begin{align*}
    f(x)-xe^{\int_0^x \frac{dt}{f(t)}}-x(c(x))
\end{align*}




\subsection{Differential equations } \label{subsec:EDP}\noindent



 Before dealing directly with the problem, let's divide it into several simplified steps. Then, with the solutions of these simplified equations, we will return to the original problem.
 
 Let us start by removing the product. Using that $1-x\leq e^{-x}$, we can concern about sequences $(p_n)_n$ such that for some $\alpha>0$: 
 \begin{align*}
     \left|p_n-\sum_{k=1}^n \exp\left\{\sum_{j=1}^k \frac{1}{p_j}\right\}\right|<\sqrt{n^{\alpha}}, \, \forall n>n_0. 
 \end{align*} Now, we can take a continuous version of the same problem by exchanging the summation with integrals, and try to find solutions $f(x)$ for the following integral inequality:
 \begin{align*}
     \left|f(x)-\int\limits_0^x dy \exp\left\{\int\limits_0^y \frac{dz}{f(z)}\right\}\right|<\sqrt{x^{\alpha}}. \,\forall x>x_0. 
 \end{align*}

 To describe the space of solutions of such integral inequality, define for every $x\in \R\setminus \{1\}$, the function:
 \begin{align*}
     \li(x)=\int\limits_{0}^x \frac{dt}{\ln{t}}.
 \end{align*} Since $\frac{1}{\ln{t}}$ have a singularity at $t=1$, for every $x>1$, we interpreted the integral as a Cauchy principal value:
 \begin{align*}
     \li(x)=\lim_{\e \to 0^+} \left(\int\limits_{0}^{1-\e} \frac{dt}{\ln{t}} + \int\limits_{1+\e}^x \frac{dt}{\ln{t}}\right).
 \end{align*}

  Notice that $\li(x)$ is a strictly increasing function in $x>1$, and strictly decreasing in $x<1$; Therefore, there exists two invertible functions, that work locally for the function $\li(x)$, one in the interval $[0,1)$ and another in the interval $(1,\infty)$. Define $\lii:\R\to (1,\infty)$ its inverse in the branch $(1,\infty)$. Using such function, we get the following.

 \begin{Lem}\label{LEM:funçãozeroli}
Consider a function $f:[0,\infty)\to \R$, $N>1$ that satisfy for every $x>0$, the following integral equation with initial conditions:
 \begin{align*}
            f(x)&=\int\limits_{0}^x dy \exp\left\{\int\limits_{0}^y \frac{dz}{f(z)}\right\}, \forall x>0.\\
            \ln{f(N)}&=C_0>0 \text{ and }f'(N)=C_1>0 \\
            2C_0&\geq C_1.
 \end{align*} Then,  the solution of the integral equation is: 
 \begin{align*}
     f(x)=e^{C_1-C_0}\left[\li\right]^{-1}((x-N+e^{C_1-C_0}\li(e^{2C_0-C_1}))e^{C_0-C_1}), \text{ for } x>0.
 \end{align*} 
 \end{Lem}

 Moreover, we have that:

 \begin{Lem}
Consider a function $f:[0,\infty)\to \R$, $N>1$ that satisfy for every $x>0$, the following integral equation:
 \begin{align*}
            f(x)&=\int\limits_{0}^x dy \exp\left\{\int\limits_{0}^y \frac{dz}{f(z)}\right\}, \forall x>0.
 \end{align*} Then, for every initial conditions that allows real solutions, there exists $c_1, c_2\in \R$ such that:
 \begin{align*}
     f(x)=\frac{1}{c_1}\left[\li\right]^{-1}(c_1(x-c_2)), \text{ for } x>0.
 \end{align*} 
 \end{Lem}
 \begin{proof}
     It is an exercise to show that $f(x)=\int\limits_{0}^x dy \exp\left\{\int\limits_{0}^y \frac{dz}{f(z)}\right\}$ as a integral of exponential function is an increasing  positive function. Moreover, whenever $f(x)$ is bounded by above, and by bellow for some constant different than zero, we can show that $f$ have a continuous second derivative. 

    So rearranging the integral equation by differentiating it, we get:  
     \begin{align*}
         f(x)=\int\limits_{0}^x dy \exp\left\{\int\limits_{0}^y \frac{dz}{f(z)}\right\}&\iff  \ln(f'(x))=\int\limits_{0}^x \frac{dz}{f(z)},\\
         &\iff f''(x)=\frac{f'(x)}{f(x)}.
     \end{align*} Integrating in $[N,x]$ we get the following differential equation with initial values:
    \begin{align*}
        f'(x)&=\ln{f(x)}+\left(C_1-C_0\right),\\
        \log(f(N))&=C_0.
    \end{align*}

     Moreover, for any function $F$, define its inverse as $F^{-1}$. Differentiating it, we get: 
    \begin{align*}
        \left[F^{-1}\right]'(x)=\frac{1}{F'(F^{-1}(x))}.  
    \end{align*} Therefore, defining:
    \begin{align*}
        F(x)&=\int\limits_0^{x} \frac{dt}{\ln{t}+(C_1-C_0)}=e^{C_0-C_1}\int\limits_0^{xe^{C_1-C_0}} \frac{du}{\ln{u}}.
    \end{align*} We finished our proof. 
 \end{proof}
 \begin{Lem}
     For every $a>0$ and $\e>0$, there exists an $n_0=n_0(a,\e)$ such that:
     \begin{align*}
         \P{P_n> (1+a)n\ln{n}}<\e. 
     \end{align*}
 \end{Lem}
 \begin{proof}
     Assume $n$ large enough such that the sequence $P_n$ have already concentrate around $\sum_{k=1}^n \lambda_{k}^{-1}$ and unfortunately $\{P_n=(1+a)n\ln{n}\}$ happens for some $a>0$. In particular, by Proposition \ref{Prop:concentrationfirt}, we can take $\delta$ small enough, such that:
     \begin{align*}
         \frac{1}{(1+\frac{3}{2}a)\ln{n}}<\frac{1-\delta}{(1+a)\ln{n}}<\lambda_n<\frac{1+\delta}{(1+a)\ln{n}}< \frac{1}{(1+\frac{1}{2}a)\ln{n}}.
     \end{align*} Using the stochastic domination of $P_n$ by a geometric of rate $\lambda_n$, we get that with high probability: 
     \begin{align*}
         P_{2n}\geq P_n+\left(1+\frac{a}{2}\right)n\ln{n} =\left(1+\frac{3}{4}a\right) 2n\ln{n}\geq \left(1+\frac{a}{2}\right)2n\ln{(2n)}. 
     \end{align*} Playing a little with the concentration of Geometric random variables, that we also get:
     \begin{align*}
         \P{P_{n+k}> \left(1+\frac{a}{4}\right)(n+k)\ln{(n+k)}, \forall n\in[n,2n]}>1-\e. 
     \end{align*} Therefore, $P_n>(1+a/4)n\ln{n}$ in this interval of size $n$; Thus, about the sum of $\lambda_n^{-1}$, we get that :
     \begin{align*}
         \sum_{k=1}^{2n} \lambda_{k}^{-1}&= \sum_{k=1}^{n} \lambda_{k}^{-1} + \lambda_n^{-1} \sum_{k=1}^n \prod_{j=1}^k \left(1-\frac{1}{P_{n+j}}\right)\\
         &\leq P_n+\sqrt{n^{\alpha}} + (1+\frac{3}{2}a)\ln{n}\sum_{k=1}^n \prod_{j=1}^k \left(1-\frac{1}{P_{n+j}}\right).
     \end{align*} In particular, we get that:
     \begin{align*}
         \sum_{k=1}^n \prod_{j=1}^k \left(1-\frac{1}{P_{n+j}}\right)&\leq \sum_{k=1}^n \exp\left\{\sum_{j=1}^n\frac{1}{P_{n+j}}\right\}\\
         &\leq \int_n^{2n} \exp\left\{\int_n^t \frac{dx}{\left(1+\frac{a}{4}\right)x\ln{x}}\right\} dt\\
         &\leq \frac{1}{\ln^{\frac{1}{(1+a/4)}}(n)} \left((1+\delta)2n\ln^{1/(1+a/4)}(2n) - (1-\delta) n\ln^{1/(1+a/4)}(n)\right)\\
         &\sim (1+3\delta)n
     \end{align*}
     
 \end{proof}
 \begin{proof}
     It is an exercise to show that $f(x)=\int\limits_{0}^x dy \exp\left\{\int\limits_{0}^y \frac{dz}{f(z)}\right\}$ as a integral of exponential function is an increasing  positive function. Moreover, whenever $f(x)$ is bounded by above, and by bellow for some constant different than zero, we can show that $f$ have a continuous second derivative. 

    So rearranging the integral equation by differentiating it, we get:  
     \begin{align*}
         f(x)=\int\limits_{0}^x dy \exp\left\{\int\limits_{0}^y \frac{dz}{f(z)}\right\}&\iff f'(x)=\exp\left\{\int\limits_{0}^x \frac{dz}{f(z)}\right\}\\
         &\iff \ln(f'(x))=\int\limits_{0}^x \frac{dz}{f(z)},\\
         &\iff  \frac{f''(x)}{f'(x)}= \frac{1}{f(x)}\\
         &\iff f''(x)=\frac{f'(x)}{f(x)}.
     \end{align*} Integrating in $[N,x]$ we get the following differential equation with initial values:
    \begin{align*}
        f'(x)&=\ln{f(x)}+\left(C_1-C_0\right),\\
        \log(f(N))&=C_0,\\
        2C_0&\geq C_1.
    \end{align*}

     Moreover, for any function $F$, define its inverse as $F^{-1}$. Differentiating it, we get: 
    \begin{align*}
        \left[F^{-1}\right]'(x)=\frac{1}{F'(F^{-1}(x))}.  
    \end{align*} Therefore, defining:
    \begin{align*}
        F(x)&=\int\limits_0^{x} \frac{dt}{\ln{t}+(C_1-C_0)}=e^{C_0-C_1}\int\limits_0^{xe^{C_1-C_0}} \frac{du}{\ln{u}}\\
        &=e^{C_0-C_1}\li(xe^{C_1-C_0}).
    \end{align*}  Again, notice that if $x>e^{C_0-C_1}$, $F(x)$ is invertible, and its inverse is a solution for the differential equation. The inverse in other hand is a positive function defined for every real number. 
    
    To get the initial conditions of the differential equation, take: 
    \begin{align*}
        f(x)= e^{C_1-C_0}\left[\li\right]^{-1}((x-N+e^{C_1-C_0}\li(e^{2C_0-C_1}))e^{C_0-C_1})
    \end{align*}
    
 \end{proof}

 \begin{Rmk}
     The condition that $2C_0\geq C_1$ is necessarily to get 
 \end{Rmk}

\begin{Lem}
    All solutions of the differential equation satisfies that:
    \begin{align*}
        \frac{f(x)-xlog(x)}{x\log(\log(x))}\to 1.
    \end{align*} 
\end{Lem}

\begin{Lem}
    Let $(q_n)_n$ be a sequence such that $\ln{q_N}=C_0$ and $\exp\left\{\sum_{j=1}^k \frac{1}{p_j}\right\}=C_1$. Consider $f(x)$ a solution of the DIV. Then $|f(n)-q_n|<n^{\alpha}$
\end{Lem} 
\begin{proof}
    It is simple to show  using induction that the discrete recurrence equation have a unique solution. 
    \begin{align*}
        q_{n+1}&=q_n+ \exp\left\{\sum_{j=1}^n \frac{1}{p_j}\right\}\\
        \ln{q_N}&=C_0, \text{ and } \exp\left\{\sum_{j=1}^N \frac{1}{q_j}\right\}=C_1.
    \end{align*}However, since this is a discrete problem it is hard to find a close formula for the solution. To overcome this difficulty, we will create a relation between such solution with the differential equation. 

    Let $(q_n)_n$ be such solution, and without loss of generality, always starting with $q_1>0$, it is simple to show that $q_n>n$. 

    To study fluctuations of such solution, let be $e_n$ be any sequence, $t>0$, and consider the sequence $h_n=q_n(1+te_n)$, We are interest to undertand, the function:
    \begin{align*}
        F(t,n)=h(n)-\sum_{k=1}^n \exp\left\{\sum_{j=1}^k \frac{1}{h_j}\right\}
    \end{align*}
    
    In particular, we have derivating in $t$ that:
    \begin{align*}
        F'(t,n)=q_ne_n- \sum_{k=1}^n \left(-\sum_{j=1}^k \frac{e_j}{h_j^2}\right) \exp\left\{\sum_{j=1}^k \frac{1}{h_j}\right\} 
    \end{align*}
    
    
    such that for some $\e>0$, we have $|e_n|<n^{1-\e}$ for every $n$.  Then define the function $h_n=q_n(1+e_n)$. Then:

    \begin{align*}
        \exp\left\{\sum_{j=1}^n \frac{1}{h_j}\right\}=
    \end{align*}
  
  
  In particular, let $h_n=q_n(1+e_n)$
\end{proof}



\begin{Prop}
    Let $(p_n)_n$, $(q_n)_n$ and $f(X)$ such that:
    \begin{align*}
        p_n&=\sum_{k=1}^{n} \prod_{j=1}^k\left(1-\frac{1}{p_j}\right)^{-1}\\
        q_n&=\sum_{k=1}^{n} \exp\left\{\sum_{j=1}^k \frac{1}{p_j}\right\}\\
       f(x)&=\int\limits_{0}^x dy \exp\left\{\int\limits_{0}^y \frac{dz}{f(z)}\right\},
    \end{align*} Also, we have that, $\ln{q_N}=\ln{p_N}=\ln{f(N)}=C_0$ and $\prod_{j=1}^k\left(1-\frac{1}{p_j}\right)^{-1}=\exp\left\{\sum_{j=1}^k \frac{1}{p_j}\right\}=f'(N)=C_1$.  Then, $|q_n-p_n|<n^{-\alpha}$ and $|q_n-f(n)|<n^{-\alpha}$.
\end{Prop}
\begin{proof}
    With the function $f(x)$ defined, construct the sequence $(f(n))_n$, notice that by definition we have that:
    \begin{align*}
        f(n)=&f(n-1)+ \int_{n-1}^{n} dy\exp\left\{\int_0^y \frac{dz}{f(z)}\right\}= f(n-1)+ e^{\int_0^{n-1} \frac{dz}{f(z)}}\int_{n-1}^{n} dy\exp\left\{\int_{n-1}^{y} \frac{dz}{f(z)}\right\}\\
        \leq& f(n-1)+ e^{\sum_{k=1}^n \frac{1}{f(k)}}  
    \end{align*} Therefore. we have that:
    \begin{align*}
        f(n)\geq f(n-1)+ e^{\sum_{k=0}^{n-1} \frac{1}{f(k)}}
    \end{align*} In that way, 
    \begin{align*}
         |f(n)- \sum_{k=1}^n e^{\sum_{j=0}^k \frac{1}{f(j)}}+\sum_{k=1}^n e^{\sum_{j=0}^k \frac{1}{f(j)}}-\sum_{k=1}^n e^{\sum_{j=1}^k \frac{1}{f(j)}}|\leq |f(n)- \sum_{k=1}^n e^{\sum_{j=1}^k \frac{1}{f(j)}}|\leq f(0)
    \end{align*}
\end{proof}



\begin{Prop}
    Let $p_n$ such that $p_n=\sum_{k=1}^{n} \prod_{j=1}^k\left(1-\frac{1}{p_j}\right)^{-1}$, then set $h_n$ such that $\left|h_n-\sum_{k=1}^{n} \prod_{j=1}^k\left(1-\frac{1}{h_j}\right)^{-1}\right|<n^{\alpha}$. Then $h_n-p_n<n^{1-\alpha}$.
\end{Prop}
\begin{proof}
     exists a function $(e_n)$ such that $h_n=p_n(1+e_n)$. 
\end{proof}

\bibliographystyle{plain}
\bibliography{ref}

\subsection{Differential equations } \label{subsec:EDP}\noindent

 The random sequences $P_n$ and $\sum_{k=1}^n \lambda_k^{-1}$ are both $\mathcal{F}_n$ measurable. This means that knowing the values of $(P_1,\cdots,P_n)$, result in knowing the value of $\sum_{k=1}^n \lambda_k^{-1}$. In particular, the event $\{\left|P_n-\sum_{k=1}^n \frac{1}{\lambda_k}\right|>n^{\frac{\alpha+1}{2}},\forall n>n_0\}$ is only satisfied for sequences where $(P_n)_n$ stays close to $\sum_{k=1}^n \prod_{j=1}^k \left(1-\frac{1}{P_j}\right)$ for every $n>n_0$, and that is not a random question.  

 Before dealing directly with the problem, let's divide it into several simplified steps. Then, with the solutions of these simplified equations, we will return to the original problem.
 
 Let us start by removing the product. Using that $1-x\leq e^{-x}$, we can concern about sequences $(p_n)_n$ such that for some $\alpha>0$: 
 \begin{align*}
     \left|p_n-\sum_{k=1}^n \exp\left\{\sum_{j=1}^k \frac{1}{p_j}\right\}\right|<\sqrt{n^{\alpha}}, \, \forall n>n_0. 
 \end{align*} Now, we can take a continuous version of the same problem by exchanging the summation with integrals, and try to find solutions $f(x)$ for the following integral inequality:
 \begin{align*}
     \left|f(x)-\int\limits_0^x dy \exp\left\{\int\limits_0^y \frac{dz}{f(z)}\right\}\right|<\sqrt{x^{\alpha}}. \,\forall x>x_0. 
 \end{align*}

 To describe the space of solutions of such integral inequality, define for every $x\in \R\setminus \{1\}$, the function:
 \begin{align*}
     \li(x)=\int\limits_{0}^x \frac{dt}{\ln{t}}.
 \end{align*} Since $\frac{1}{\ln{t}}$ have a singularity at $t=1$, for every $x>1$, we interpreted the integral as a Cauchy principal value:
 \begin{align*}
     \li(x)=\lim_{\e \to 0^+} \left(\int\limits_{0}^{1-\e} \frac{dt}{\ln{t}} + \int\limits_{1+\e}^x \frac{dt}{\ln{t}}\right).
 \end{align*}

  Note that $\li(x)$ is a strictly increasing function in $x>1$, therefore it is invertible in this interval. In particular define $\lii:\R\to (1,\infty)$ its inverse. Using such function, we get the following.

 
 \begin{Lem}\label{LEM:funçãozeroli}
Consider a function $f:[0,\infty)\to \R$, that satisfy for every $x>0$, and $C_0>0$ the following integral equation with initial conditions:
 \begin{align*}
            f(x)&=\int\limits_{0}^x dy \exp\left\{\int\limits_{0}^y \frac{dz}{f(z)}\right\}, \forall x>0.\\
            \ln{f(0)}&=f'(0)=C_0>0; 
 \end{align*} Then, for every $x>0$, $f(x)$ is infinitely differentiable. Let $\mu=\lii[0]$ the Ramanujan–Soldner constant, then, we get that: 
 \begin{align*}
     f(x)=\left[\li\right]^{-1}(x+\mu-e^{C_0}), \text{ for } x>0.
 \end{align*} 
 \end{Lem}
 \begin{proof}
     Assume that $f(x)=\int\limits_{0}^x dy \exp\left\{\int\limits_{0}^y \frac{dz}{f(z)}\right\}$ is infinitely differentiable for every $x>0$. Then, we get that:
     \begin{align*}
         f'(x)=\exp\left\{\int\limits_{0}^x \frac{dz}{f(z)}\right\}
     \end{align*}Since, the exponential is always positive, we get that:
     \begin{align*}
         \ln(f'(x))=\int\limits_{0}^x \frac{dz}{f(z)}, 
     \end{align*}that is also differentiable, leading to the differential equation:
     \begin{align*}
        \frac{f''(x)}{f'(x)}&= \frac{1}{f(x)}, \text{ that implies }\\
        f''(x)&=\frac{f'(x)}{f(x)}.
    \end{align*} Integrating in $[0,x]$ we get the following differential equation with initial values:
    \begin{align*}
        f'(x)&=\ln{f(x)},\\
        f'(0)&=C_0>0. 
    \end{align*}

     Moreover, for any function $F$, define its inverse as $F^{-1}$. Differentiating it, we get: 
    \begin{align*}
        \left[F^{-1}\right]'(x)=\frac{1}{F'(F^{-1}(x))}.  
    \end{align*} Therefore, when $F(x)=\li(x+\mu-e^{C_0})$, defining the inverse when $x+\mu-e^{C_0}>1$, we get:
    \begin{align*}
         \left[F^{-1}\right]'(x)= \ln{F^{-1}(x)}. 
    \end{align*}Moreover, 
    \begin{align*}
         \left[F^{-1}\right]'(0)= \ln{F^{-1}(0)}=\ln{e^{C_0}}=C_0>0. 
    \end{align*} Therefore, the unique solution for the problem with initial value is the infinitely differentiable function $f(x)=\left[\li\right]^{-1}(x+\mu-e^{C_0})$, as desired.
    
 \end{proof}

 
 \begin{Lem}\label{LEM:funçãozerol2i}
Consider a function $f:[0,\infty)\to \R$, that satisfy for every $x>0$, $C_0>0$ and $C_1>0$ the following integral equation with initial conditions:
 \begin{align*}
            f(x)&=\int\limits_{0}^x dy \exp\left\{\int\limits_{0}^y \frac{dz}{f(z)}\right\}, \forall x>0.\\
            \ln{f(0)}&=C_0>0\\
            f'(0)&=C_1>0; 
 \end{align*} Then, for every $x>0$, $f(x)$ is infinitely differentiable. Let $\mu=\lii[0]$ the Ramanujan–Soldner constant, then, we get that: 
 \begin{align*}
     f(x)=\left[\int\limits_0^{x+\mu e^{C_0-C_1}-e^{2C_1-C_0}} \frac{dt}{\ln{t}+(C_1-C_0)}\right]^{-1}, \text{ for } x>0.
 \end{align*} 
 \end{Lem}
 \begin{proof}
    In this problem, we are interesting in solve the following differential equation with initial values: 
    \begin{align*}
        f'(x)&=\ln{f(x)}+(C_1-C_0)\\
        f'(0)&=C_1.
    \end{align*}

    For this, define
    \begin{align*}
        F(x)=\int\limits_0^{x} \frac{dt}{\ln{t}+(C_1-C_0)}=e^{C_0-C_1}\int\limits_0^{xe^{C_1-C_0}} \frac{du}{\ln{u}}.
    \end{align*}  Notice that when $t=e^{C_1-C_0}$ the function has a singularity, therefore for every $x> e^{C_1-C_0}$, we define the integral as the Cauchy principal value.  
    
    Moreover, for every $x>e^{C_1-C_0}$, $F(x)$ is strictly increasing, so we can define $F^{-1}$ as its inverse.  Differentiating $F^{-1}$, we get: 
    \begin{align*}
        \left[F^{-1}\right]'(x)= \ln{F^{-1}(x)}+(C_0-C_1). 
    \end{align*} Therefore, $F^{-1}$ is one possible solution. To get the boundary conditions, we define $f(x)=\left[F^{-1}\right]\left(x+\mu e^{C_0-C_1}-e^{2C_1-C_0}\right)$.
 \end{proof}


\subsection{First Concentration result}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\begin{proof}
    The proof consists in finding an upper and lower bound for the fraction. Fixing any integer $k>1$ and $\delta>0$, using the fact that $f(x)\in \SV$, we can find $x_0(\delta,k)$ such that for every $x>x_0$:
    \begin{align}\label{eq:lambdauniformslowlyvaring}
        1+\delta\geq  \frac{f\left(x\frac{j}{k}\right)}{f(x)}\geq  1-\delta, \quad \forall j\in\{1,\cdots,k\}.
    \end{align} Thus, by the monotonicity of $f(x)$, we have that:  
    \begin{align*}
        \frac{\int\limits _{0}^{x} f(y)dy}{xf(x)}&= \sum_{j=0}^{k-1} \frac{1}{xf(x)}\int\limits_{\frac{j}{k}x}^{\frac{j+1}{k}x} f(y)dy \\
        &\leq \sum_{j=0}^{k-1} \frac{xf\left(x\frac{j+1}{k}\right)}{k xf(x)}\leq 1+\delta.
    \end{align*} For the other side, assuming without loss of generality that $\delta<\frac{1}{2}$, which implies that $\frac{1+\delta}{k}<1$ since $k\geq 2$. Then, notice that:
    \begin{align*}
        \frac{\int\limits_{0}^{x} f(y)dy}{xf(x)}&\geq \frac{\int\limits_0^{\frac{x}{k}} f(y)dy}{xf(x)}+ \frac{k-1}{k}(1-\delta) \\
        &= \frac{f\left(\frac{x}{k} \right)}{kf(x)} \frac{\int\limits_0^{\frac{x}{k}} f(y)dy}{\frac{x}{k}f\left(\frac{x}{k}\right)}+ \frac{k-1}{k}(1-\delta)\\
        &\geq (1-\delta)+ \frac{1-\delta}{k} \left(-1+\frac{\int\limits_0^{\frac{x}{k}} f(y)dy}{\frac{x}{k}f\left(\frac{x}{k}\right)}\right).
    \end{align*} In particular, with $x=x_0k^n$, we get that: 
    \begin{align}\label{eq:boundswithk^ninthekaramatarate}
        \frac{\int\limits _{0}^{x} f(y)dy}{xf(x)}&\geq (1-\delta)+ \delta \sum_{j=1}^n \left(\frac{1-\delta}{k}\right)^j + \left(\frac{1-\delta}{k}\right)^{n+1}\frac{\int\limits_0^{{x_0}} f(y)dy}{x_0f\left(x_0\right)}.
    \end{align}Which implies, for $\delta<\frac{1}{2}$, and $k\geq 2$ that:
    \begin{align*}
        \liminf_{x\to \infty }\frac{\int\limits _{0}^{x} f(y)dy}{xf(x)}\geq 1-\delta\left(1+\frac{1}{1-\frac{1-\delta}{k}}\right)\geq 1-2\delta.
    \end{align*}Concluding the proposition. 
\end{proof}


The above process have a connection with prime numbers, notice that given the first $n$ primes $(p_1,...,p_n)$, associated with each prime $p_j$, we have the set of multiples ${M}_j=\{kp_j: k\in \N\}$, it is classical that the union of the multiples is not $\N$, that is $\bigcup_{j=1}^n {M}_j\neq \N$, thus there exists always a minimal element that will be our next prime $p_{n+1}$. In this paper, with a set of the first elements $(P_1,\cdots,P_n)$, each with its own independent renewal set $\mathcal{M}_j$ of multiples,   

so the process do not concerns about the points achieved by the renewal, but instead it looks to the first point not taken. In such point,  so we will not be concern  and we will get concentration results that resembles the prime number theorem. 


Since the minimun of geometric randon variables are also geometric4

To justify the name of random primes, fixed any $n\in \N$ and flip a coin with parameter $\frac{1}{n}$ for each natural, if the coin is head, we say that the number is multiple of $n$, if it is tail, we say that the number is not multiple. In this notation, the random variable $P_k$ is the first point that is not multiple of nether primes $P_1,P_2,...,P_{k-1}$. 

Let $(p_n)_n$ be the sequence of primes, and notice that $\Ex{P_n|P_{n-1}=p_{n-1},...,P_1=p_1}=p_n$. In the sense that the best guess of $(P_n)_n$ maybe the prime numbers $(p_n)_n$. Not only, this is true, we have
\begin{Thm}
For every $\e>0$, we have that:
\begin{align*}
\lim_{n\to \infty} \P{n\ln^{(1-\e)}(n)<P_n<(1+\e)n\ln{(n)}}=1
\end{align*}
\end{Thm}

???
\begin{Thm}
$\lim_{x\to \infty} \ln{(x)}\P{x\text{ be prime}}=1$. 
\end{Thm}

\begin{Cor}
There are finitely many primes of the form $2^{2^k}+1$, $2^{k ^2}+1$. Since, the natural numbers are one sample of my space, we have that:
\begin{align}
\P{\text{Existem finitos numeros de Fermart}}=1.
\end{align}
\end{Cor}
